Intrinsic Dimension Estimation Using Wasserstein Distances

It has long been thought that high-dimensional data encountered in many practical machine learning tasks have low-dimensional structure, i.e., the manifold hypothesis holds. A natural question, thus, is to estimate the intrinsic dimension of a given population distribution from a finite sample. We introduce a new estimator of the intrinsic dimension and provide finite sample, non-asymptotic guarantees. We then apply our techniques to get new sample complexity bounds for Generative Adversarial Networks (GANs) depending only on the intrinsic dimension of the data.

==> secEmpirical.tex <==
\section{Experiments}
In this section, we provide empirical evidence for the success of our estimator through a number of experiments.  We note that while \Cref{thm:estimator} examines the case of samples of two sizes ($n$ and $\alpha n$), we find that the estimator is more stable if we use several different sample sizes and find the slope of the resulting regression line between $\log_2 n$ and $\log_2 W_1(P_n, P_n')$.  In our experiments, we use $n  = 2^k$ for $k \in \{5,6,7,8,9,10\}$.  In order to compute $W_1(P_n, P_n')$, we could use either the Hungarian Matching algorithm or the network simplex algorithm, both described in detail in \citep{peyre2019computational}; however, this is relatively slow, taking $O(n^3\log n)$ time for each $n = 2^k$.  As this slow time is prohibitively expensive, we instead use the Sinkhorn algorithm for computing the entropically regularized optimal transport cost \citep{cuturi2013}.  We know from \citep{altschuler2017near} that we can approximate $W_1(P_n, P_n')$ up to a factor of $\epsilon$ in time $O\left(n^2 \log n \epsilon^{-3}\right)$.  For most of our experiments, we do not bother to approximate the intrinsic metric as we find that it does not affect the dimension estimation \adamcomment{Run some experiments to demonstrate this}.  In our last experiment, with the MNIST data set, we do, however, need this step.  While the proof uses graphs constructed by connection $\epsilon$-balls, we instead use a nearest neighbor rule where a data point $X_i$ is connected to each of its $k$ nearest neighbors.  As remarked in \citep{Bernstein00}, this difference is not important for large $n$, but, computationally, we find that it leads to better-connected graphs.  We now discuss our experiments in detail. \adamcomment{Cite Julia Optimal Transport}.

First, we consider a very simple toy setting where $\pp$ is the uniform distribution on an imbedded unit sphere.  The intrinsic dimension $d$ is the dimension of the unit sphere, which is then imbedded with a high degree polynomial mapping into $\rr^D$ for some large $D$.  We generate two datasets each of size $n = 2^k$ for $5 \leq k \leq 10$, compute the Wasserstein distance between them and then plot $\log_2 W_1(P_n, P_n')$ against $\log_2 n$.  A typical plot looks like \Cref{fig:sample}.

\begin{figure}
    \centering
    \includegraphics[width=.8\textwidth]{Figures/Sample Plot.png}
    \caption{Plot of $\log W_1(P_n, P_n')$ against $\log n$.  Here $\pp$ is uniform on the sphere $S^8$ imbedded in $\rr^{100}$ through a high degree, polynomial imbedding.}
    \label{fig:sample}
\end{figure}
We examine such plots for intrinsic dimension $5 \leq d \leq 25$ and compare the resulting estimate to the MLE dimension estimator of \citep{levina2004maximum} in \Cref{fig:changed}.

\begin{figure}
    \centering
    \includegraphics[width=.8\textwidth]{Figures/Comparison with MLE.png}
    \caption{Graph of estimated intrinsic dimension against actual intrinsic dimension of spheres imbedded in $\rr^D$ under a high degree, polynomial imbedding.  We compare our estimator to that of \citep{levina2004maximum}.}
    \label{fig:changed}
\end{figure}
We further examine the effect that increasing the ambient dimension has on our estimator in \Cref{fig:changeD}.  We note that it has no effect.
\begin{figure}
    \centering
    \includegraphics[width=.8\textwidth]{Figures/MLEComparison2.png}
    \caption{We plot the estimated intrinsic dimension against the ambient dimension and notice that the ambient dimension has no effect on the estimator.  We compare this to the MLE estimator of \citep{levina2004maximum}.}
    \label{fig:changeD}
\end{figure}
We now consider real data sets.  We estimate the dimension of the classic Swiss Roll data set \citep{tenenbaum2000} and estimate a dimension of $2.4$ (the real dimension is $2$).  We then apply our dimension estimator to each digit in the MNIST data set \adamcomment{Include reference}, and summarize the results in \Cref{fig:mnist}.
\begin{figure}
    \centering
    \includegraphics[width=.8\textwidth]{Figures/MNISTDims.png}
    \caption{Summary of the estimated intrinsic dimensions of MNIST digits, grouped by digit.  We use two different estimates, one with an entropic regularization of $.1$ and the other with an entropic regularization of $.05$.  In the former case, we run Sinkhorn for 10k iterations and in the latter we run Sinkhorn for 30k iterations.}
    \label{fig:mnist}
\end{figure}

Our results suggest that previous estimates of the intrinsic dimensionality of MNIST digits may be too large.

